ScribbleGen: Generative Data Augmentation Improves Scribble-supervised Semantic Segmentation

Recent advances in generative models, such as diffusion models, have made generating high-quality synthetic images widely accessible. Prior works have shown that training on synthetic images improves many perception tasks, such as image classification, object detection, and semantic segmentation. We are the first to explore generative data augmentations for scribble-supervised semantic segmentation. We propose ScribbleGen, a generative data augmentation method that leverages a ControlNet diffusion model conditioned on semantic scribbles to produce high-quality training data. However, naive implementations of generative data augmentations may inadvertently harm the performance of the downstream segmentor rather than improve it. We leverage classifier-free diffusion guidance to enforce class consistency and introduce encode ratios to trade off data diversity for data realism. Using the guidance scale and encode ratio, we can generate a spectrum of high-quality training images. We propose multiple augmentation schemes and find that these schemes significantly impact model performance, especially in the low-data regime. Our framework further reduces the gap between the performance of scribble-supervised segmentation and that of fully-supervised segmentation. We also show that our framework significantly improves segmentation performance on small datasets, even surpassing fully-supervised segmentation. The code is available at https://github.com/mengtang-lab/scribblegen.

==> sec/2_relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}

\paragraph{Synthetic training data}
% @jieke
% DatasetGAN \cite{Datasetgan}
% ImageNet \cite{syntheticimagenet}
% DiffusionEngine (object detection) \cite{DiffusionEngine}
% FreeMask (segmentation on ADE): \cite{freemask}
% D3S \cite{kattakinda2022invariant}
Numerous efforts have been dedicated to leveraging synthetic data for training perception models. 
IT-GAN \cite{itgan} shows that GAN-generated samples can help classification models learn faster and improve performance. 
DatasetGAN \cite{Datasetgan} and BigDatasetGAN \cite{Li_2022_CVPR} employ GANs \cite{stylegan, biggan} for jointly generating synthetic images and their corresponding labels for segmentation tasks.

Recent advances in diffusion models have brought notable stability during training, robust synthesis capabilities \cite{dhariwal2021diffusion}, and enhanced controllability \cite{controlnet}. 
As a result, there has been a significant shift towards the use of diffusion models for data synthesis, including for image classification \cite{syntheticimagenet, kattakinda2022invariant}, object detection \cite{DiffusionEngine}, instance segmentation \cite{xie2023mosaicfusion}, and semantic segmentation \cite{nguyen2023dataset, wu2023datasetdm, freemask}. 
For example, by fine-tuning an Imagen \cite{imagen} model on ImageNet \cite{imagenet}, \cite{syntheticimagenet} generates synthetic images from text prompts to improve the performance of image classification. 
Similarly, D3S \cite{kattakinda2022invariant} introduces a novel synthetic dataset specially designed to mitigate the foreground and background biases prevalent in real images. 
Dataset Diffusion \cite{nguyen2023dataset} and DatasetDM \cite{wu2023datasetdm} jointly generate synthetic images and associated mask annotation, akin to DatasetGAN, using a StableDiffusion \cite{latentdiffusion} image-generative model.
FreeMask \cite{freemask} utilizes FreestyleNet \cite{freestyle} to synthesize images conditioned on full mask annotations.

Our work diverges from these initiatives by focusing on sparse labels (e.g., scribbles) from real images as generative conditions, encouraging the creation of realistic and diverse synthetic images. 
While FreeMask \cite{freemask} similarly conditions synthetic images on real data annotations, our method uses sparse rather than dense annotations, allowing for broader applications where dense labeling is expensive.

\paragraph{Guidance in Diffusion models}
%Image-generative models have been an area of active research over the past decade, where the task is to synthesize high-quality images.Some of the earlier works in generative models include Generative Adversarial Networks (GANs) \cite{gans, stylegan, improvestylegan, biggan}, Variational AutoEncoders (VAEs) \cite{vae, vqvae}, and flow-based models \cite{glow}. However, recent work in Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ddpm}\tao{todo} shows state-of-the-art performance \cite{latentdiffusion, imagen}.Whereas GANs require reaching an equilibrium between a generative model and a discriminative model, DDPMs achieve their results by iterative denoising of an initial input into an image.

%\tao{TODO}For many applications, however, simply synthesizing realistic images unconditionally, is insufficient.
%These generative models are made most effective by the addition of multi-modal conditioning input such as text prompts or semantic masks to control synthesis \cite{conditionalgan, conditionalvae, latentdiffusion, ramesh2022hierarchical}.
%Conditioned synthesis from images is still very active with methods for GANs \cite{spade, wang2021dg} and especially diffusion models \cite{controlnet, semanticdiffusion, gligen, freestyle} showing very promising results.
%
%\tao{todo}Related to conditioned diffusion is the topic of guided diffusion, which seeks to further guide the synthesis process in the latent space.\cite{dhariwal2021diffusion} accomplishes guidance with the gradients of a classification model, whereas \cite{classifierfree, selfguided} show that guidance can be accomplished without an auxiliary model or extra annotation.
%In this paper, we leverage guided diffusion models for their superior generation performance \cite{dhariwal2021diffusion}.

Diffusion models excel in various tasks due to their controllability~\cite{controlnet}. 
They're used to generate image content~\cite{ddpm}, image layout~\cite{latentdiffusion,selfguided,meng2021sdedit}, audio content~\cite{liu2023audioldm}, human motion~\cite{tevet2022human_mdm}, etc. 
Guidance signals can also be incorporated to enhance image fidelity~\cite{dhariwal2021diffusion, classifierfree} relative to unconditional generation.
It has been shown that diffusion models can be guided by pretraining a noisy-data-based classifier, known as Classifier-guidance~\cite{dhariwal2021diffusion}. 
On the other hand, classifier-free guidance~\cite{classifierfree} removes the need for extra pretraining by randomly dropping out the guidance signal during training. 
We develop a framework that utilizes classifier-free guidance for generative data augmentation to improve scribble-based segmentation.  

\paragraph{Weakly-supervised segmentation}
Weakly-supervised segmentation methods use weak annotations rather than full segmentation masks to train segmentation networks for images~\cite{rloss,ke2021universal,chang2020weakly,TEL,AGMM,Groupvit} or point clouds~\cite{scribblelidar}. 
Forms of weak annotations include points~\cite{whatsthepoint,rloss,AGMM}, scribbles~\cite{rloss,TEL,AGMM}, bounding boxes~\cite{simpledoesit}, image-level tags \cite{chang2020weakly}, and text~\cite{Groupvit}. 
These methods can be roughly categorized into two groups. 
The first group proposes various unsupervised or semi-supervised losses such as entropy loss~\cite{changmixup}, CRF loss~\cite{rloss}, and contrastive-learning losses~\cite{ke2021universal}. 
The second group iteratively refines full-mask pseudo-labels~\cite {simpledoesit,scribblesup} during training to mimic full supervision. 
Many weakly-supervised approaches rely on class activation maps (CAMs)~\cite{CAM,changmixup} that gives localization cues from classification networks. 
Our generative data augmentation approach complements any existing weakly-supervised segmentation methods, as we show improved performance of several methods with our synthetic data.

Weak annotations can also be provided as input for segmentation networks at test time for interactive segmentation~\cite{deepgrabcut,sam}. 
For example, Segment Anything~\cite{sam} allows prompts including clicks, bounding boxes, masks, or text. 
While Segment Anything~\cite{sam} provides many masks in a semi-automatic way for training interactive segmentation, we focus on synthetic image synthesis for training weakly-supervised segmentation.


==> sec/X_Discriminator_guidance.tex <==
\clearpage
\section{Discriminator guidance}

% The \textit{discriminator guidance} \cite{discriminatorguidance} is originally stated in SDE framework as 
% $$ \dd \bx_t = [f(\bx_t) - g^2(t) (s_{\theta_\infty} + c_{\theta_\infty}) (\bx_t, t) ] \dd \bar{t} + g(t) \dd \bar{\mathbf{w}}_t $$
% where $s_{\theta_\infty}$ is the score function and $c_{\theta_\infty}$ is the discriminator guidance defined by
% $$ c_{\theta_\infty} \approx \nabla \log \frac{d_{\boldsymbol{\phi}}\left(\mathbf{x}_t, t\right)}{1-d_{\boldsymbol{\phi}}\left(\mathbf{x}_t, t\right)} $$
% where $d_{\boldsymbol{\phi}}$ is a discriminator that outputs classification probabilities for real and synthetic classes.

\jieke{Notations and wording will be modified later.}

\jieke{TODO: move dg to xt term.}


\begin{algorithm}[h!]
\caption{Conditional DDIM sampling with guidance scale $w$, encode ratio $\lambda$, discriminator guidance scale $\psi$}
\label{alg:sampling-dg}
\DontPrintSemicolon
% \Require{$\alpha$: noise schedule}
\Require{$q_\sigma$: forward process}
\Require{$d_\phi$: discriminator}
\Require{$\bxref$: a reference image}
\Require{$w\ge0$: guidance scale}
\Require{$\lambda\in [0, 1]$: encode ratio}
% \Require{$\sigma\ge0$: DDIM stochasticity parameter}
% \Require{$T$: maximum number of forward diffusion process steps}
\Require{$N\in\{1,\ldots,T\}$: number of reverse diffusion process steps}
\Require{$c_t$ and $c_s$: text prompt and scribble conditioning}
% \Require{$\tilde{c}$: learned unconditional embedding}
$\bepsilon\sim\mathcal{N}(0,I)$\;
$\tau=[\lfloor\frac{\lambda T}{N}n\rfloor:0\le n\le N]$\;
\Comment{Note if $\lambda=1$ then $\bx_{\tau_N}\sim\mathcal{N}(0,I)$}
$\bx_{\tau_N}=\sqrt{\alpha_{\tau_N}}\bxref+\sqrt{1-\alpha_{\tau_N}}\bepsilon$\;
\For{$i=N$ to $1$}{
    \Comment{Predict added noise using diffusion guidance (\ref{eq:cfg-custom})}
    \mbox{$\begin{aligned}
        \tilde{\bepsilon}_{\tau_{i}} = &(1+w)\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_{i}},c_t,c_s) \\ &- w\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_i}, c_t,\tilde{c}_s)
    \end{aligned}$}\;%\vspace{-.9em}
    \Comment{\mbox{Accelerated DDIM sampling (\ref{eq:ddim-sampling})}}
    $\hat{\bx}_0=(\bx_{\tau_i}-\sqrt{1-\alpha_{\tau_i}}\cdot\tilde{\bepsilon}_{\tau_i})/\sqrt{\alpha_{\tau_i}}$\;
    \uIf{$i=1$}{
        $\bx_{0}\sim \mathcal{N}(\hat{\bx}_{0},\sigma^2_{\tau_1}I)$\;
    }
    \Else{
        % $\bx_{\tau_{i-1}}\sim q_\sigma(\bx_{\tau_{i-1}}|\bx_{\tau_i},\hat{\bx}_0)$\;
        $\bx_{\tau_{i-1}} = \sqrt{\alpha_{\tau_{i-1}}} \hat{\bx_0} + \sqrt{1-\alpha_{\tau_{i-1}} -\sigma_{\tau_i}^2} \cdot \epsilon_\theta (\bx_{\tau_i}) + \sigma_{\tau_i} \epsilon_{\tau_i} + \psi c_{\theta_\infty}(\bx_{\tau_i}, t)$
    }
    % $\bx_{\tau_{i-1}}^{(\mathrm{cond})}\sim p_\theta^{(\tau_{i-1})}(\bx_{\tau_{i-1}}|\bx_{\tau_i},c_t,c_s)$\;
    % \psi c_{\theta_\infty}(\bx_{\tau_i}, t)
}
\Return $\bx_0$\;
\end{algorithm}

\paragraph{}
How to add the discriminator guidance (DG) term on top of classifier free guidance (CFG). In CFG, it uses model $\bepsilon_\theta^{(\tau_{i})}(\bx_t,c_t,c_s)$ to approximate the sum of mean of $q_\sigma$ in equation \ref{eqn2:qsigma} and classifier guidance (CG). Since DG can be added on top of CG by algorithm 2 in \cite{discriminatorguidance}, we can add the discriminator guidance
$$c_{\theta_\infty} \approx \grad \log \frac{d_\phi(\bx, t)}{1 - d_\phi(\bx, t)}$$
to the conditional model to get $\bepsilon_\theta^{(\tau_{i})}(\bx_t,c_t,c_s) + \psi c_{\theta_\infty}(\bx_t, t)$, where $\psi$ is the scale for discriminator guidance.
So the sampling process should become $\tilde{\bepsilon}_{\tau_{i}} = (1+w)(\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_{i}},c_t,c_s) + \psi c_{\theta_\infty}(\bx_{\tau_i}, t)) - w\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_i}, c_t,\tilde{c}_s)$.

\begin{algorithm}[h!]
\caption{Discriminator training}
\label{alg:dis-training}
\DontPrintSemicolon
% \Require{$\alpha$: noise schedule}
\Require{$w\ge0$: guidance scale}
\Require{$\lambda\in [0, 1]$: encode ratio}
% \Require{$\sigma\ge0$: DDIM stochasticity parameter}
% \Require{$T$: maximum number of forward diffusion process steps}

\Require{$\mathcal{D}$ real images}
\Require{$\mathcal{G}$ synthetic images}
\Require{$\Lambda$: time-weighting function}

\While{not converged}{
    $\tau=[\lfloor\frac{\lambda T}{N}n\rfloor:0\le n\le N]$\; \\
    sample $\{\bx^{(1)}, \dots, \bx^{(B/2)}\}$ from $\mathcal{D}$; \\
    sample $\{\bx^{(B/2)}, \dots, \bx^{(B)}\}$ from $\mathcal{G}$; \\
    sample $\tau_i$ from $[\lfloor\frac{\lambda T}{N}n\rfloor:0\le n\le N]$; \\
    \mbox{$\forall j=1,\dots,B: \bx_{\tau_N}^{(B)} = \sqrt{\alpha_{\tau_N}}\bx^{(j)} + \sqrt{1-\alpha_{\tau_N}}\bepsilon$}; \\
    $\forall j=1,\dots,B:$ diffuse to get $\bx_{\tau_i}^{(j)}$ with \autoref{alg:sampling}; \\
    $\hat{\mathcal{L}}_\phi = -\sum_{i=1}^{B/2} \Lambda(\tau_i) \log d_\phi(\bx_{\tau_i}^{(j)}, \tau_i)
        - \sum_{i=B/2}^{B} \Lambda(\tau_i) \log(1 - d_{\phi}(\bx_{\tau_i}^{(j)}))$; \\
    % \mbox{
    % $\begin{aligned}
    %     \hat{\mathcal{L}}_\phi = &-\sum_{i=1}^{B/2} \Lambda(\tau_i) \log d_\phi(\bx_{\tau_i}^{(j)}, \tau_i) \\
    %     &- \sum_{i=B/2}^{B} \Lambda(\tau_i) \log (1 - d_\phi(\bx_{\tau_i}^{(j)}))
    % \end{aligned}$
    % }
    \mbox{$\phi \leftarrow \phi - \pdv{\hat{\mathcal{L}}_\phi}{\phi}$}; \\
}


% \Require{$\tilde{c}$: learned unconditional embedding}
% $\bepsilon\sim\mathcal{N}(0,I)$\;

% \Comment{Note if $\lambda=1$ then $\bx_{\tau_N}\sim\mathcal{N}(0,I)$}
% $\bx_{\tau_N}=\sqrt{\alpha_{\tau_N}}\bxref+\sqrt{1-\alpha_{\tau_N}}\bepsilon$\;
% \For{$i=N$ to $1$}{
%     \Comment{Predict added noise using diffusion guidance (\ref{eq:cfg-custom})}
%     \mbox{$\begin{aligned}
%         \tilde{\bepsilon}_{\tau_{i}} = &(1+w)(\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_{i}},c_t,c_s) + \psi c_{\theta_\infty}(\bx_{\tau_i}, t)) \\ &- w\bepsilon_\theta^{(\tau_{i})}(\bx_{\tau_i}, c_t,\tilde{c}_s)
%     \end{aligned}$}\;%\vspace{-.9em}
%     \Comment{\mbox{Accelerated DDIM sampling (\ref{eq:ddim-sampling})}}
%     $\hat{\bx}_0=(\bx_{\tau_i}-\sqrt{1-\alpha_{\tau_i}}\cdot\tilde{\bepsilon}_{\tau_i})/\sqrt{\alpha_{\tau_i}}$\;
%     \uIf{$i=1$}{
%         $\bx_{0}\sim \mathcal{N}(\hat{\bx}_{0},\sigma^2_{\tau_1}I)$\;
%     }
%     \Else{
%         $\bx_{\tau_{i-1}}\sim q_\sigma(\bx_{\tau_{i-1}}|\bx_{\tau_i},\hat{\bx}_0)$\;
%     }
    % $\bx_{\tau_{i-1}}^{(\mathrm{cond})}\sim p_\theta^{(\tau_{i-1})}(\bx_{\tau_{i-1}}|\bx_{\tau_i},c_t,c_s)$\;
\end{algorithm}




